Unimodular Proca Theory: Breaking the U(1) gauge symmetry of unimodular gravity via a mass term

We study the Hamiltonian structure of unimodular-like theories, where the cosmological constant (or other supposed constants of nature) are demoted from fixed parameters to classical constants of motion. No new local degrees of freedom are present as a result of a $U(1)$ gauge invariance of the theory. Hamiltonian analysis of the action reveals that the only possible gauge fixing that can be enforced is setting the spatial components of the four-volume time vector ${\cal T}^{i}\approx0$. As a consequence of this, the gauge-fixed unimodular path integral is equivalent to the minisuperspace unimodular path integral. However, should we break the $U(1)$ gauge invariance, two things happen: a massless propagating degree of freedom appears, and the (gauge-invariant) zero-mode receives modified dynamics. The implications are investigated, with the phenomenology depending crucially on the target ``constant''.

==> removedthings.tex <==

\section{Explicit solutions}
The EOM can be derived:
\begin{eqnarray}
    \partial_\mu \rho_\Lambda&=&M^6T_\mu=M^6g_{\mu\nu}\frac{{\cal{T}_\mu }}{\sqrt{-g}}\\
    \partial _\mu \cal{T}^\mu&=&\sqrt{-g}
\end{eqnarray}
[find the modified Einstein equation as well?]
which leads to an inhomogeneous equation for $\Lambda$:
\begin{equation}
    \Box \rho_\Lambda=\frac{1}{\sqrt{-g}}\partial _\mu (\sqrt{-g}\partial^\mu\rho_\Lambda)=M^6
\end{equation}
[fix proportionality constants if needed]
The zero mode equations are affected of course, but once solved they leave a massless local particle, the Lambdon. 

Specifically we can write:
\begin{equation}
    \rho_\Lambda=\rho_{\Lambda 0} +
    \rho_{\Lambda 1}
\end{equation}
where $\rho_{\Lambda 0}$ is a particular solution without any spatial variation (a zero model). For example in FRW backgrounds we have:
\begin{equation}
    \ddot \rho_{\Lambda 0}+3\frac{\dot a}{a}\dot \rho_{\Lambda 0}=M^6. 
\end{equation}
The $\rho_{\Lambda 1}$ are then massless waves propagating on this background. They represent the local degree of freedom we had predicted from our Hamiltonian analysis.  


Hence we have a local massless free propagating mode plus a global driven zero mode. In this case the latter is a disaster since we would get
\begin{equation}
    \rho_{\Lambda 0}=\frac{M^6}{2}t^2
\end{equation}
with hardly a commendable phenomenology. But this is just a start... (Do we need to play with a more general potential $V=V(T_\mu T^\mu)$ generalizing the quadratic potential?) 

We could do this for any other ``constant'', namely the Planck mass, etc, with similar effects. What effect would this have on the sequester?
